Byzantine-tolerant Distributed Grow-only Sets: Specification and Applications

In order to formalize Distributed Ledger Technologies and their interconnections, a recent line of research work has formulated the notion of Distributed Ledger Object (DLO), which is a concurrent object that maintains a totally ordered sequence of records, abstracting blockchains and distributed ledgers. Through DLO, the Atomic Appends problem, intended as the need of a primitive able to append multiple records to distinct ledgers in an atomic way, is studied as a basic interconnection problem among ledgers. In this work, we propose the Distributed Grow-only Set object (DSO), which instead of maintaining a sequence of records, as in a DLO, maintains a set of records in an immutable way: only Add and Get operations are provided. This object is inspired by the Grow-only Set (G-Set) data type which is part of the Conflict-free Replicated Data Types. We formally specify the object and we provide a consensus-free Byzantine-tolerant implementation that guarantees eventual consistency. We then use our Byzantine-tolerant DSO (BDSO) implementation to provide consensus-free algorithmic solutions to the Atomic Appends and Atomic Adds (the analogous problem of atomic appends applied on G-Sets) problems, as well as to construct consensus-free Single-Writer BDLOs. We believe that the BDSO has applications beyond the above-mentioned problems.

==> introduction_old.tex <==
\remove{ %% removing intro
%\input{introduction_v1}
We are living a huge hype of the so-called crypto-currrencies, and their technological support, the blockchain \cite{N08bitcoin}. It is claimed that using crypto-currencies and public distributed ledgers (i.e., public blockchains) will liberate stakeholder owners from centralized trusted authorities \cite{NYT-blockchain}.
%we are going to be free of the control of government and banks \cite{NYT-blockchain}. 
Moreover, it is believed that there is the opportunity of becoming rich by mining coins, speculating with them, or even launching your own coin 
(i.e., with an initial coin offering, ICO).

%But how this hype was nurtured and why it led to a wild adoption of cryptocurrencies? 
Cryptocurrencies were first introduced in 2009 by Satoshi Nakamoto \cite{N08bitcoin}. 
In his paper, Nakamoto introduced the first algorithm 
that allowed economic transactions to be accomplished between peers without the need of 
a central authority. An initial analysis of the security of the protocol was presented in  \cite{N08bitcoin},
although a more formal and thorough analysis was developed by Garay, Kiayias, and Leonardos in \cite{GKL15}. 
In that paper the authors define and prove two fundamental properties of the blockchain implementation 
behind bitcoin: $(i)$ \textit{common-prefix}, and $(ii)$ \textit{quality of chain}.

Although the recent popularity of distributed ledger technology (DLT), or blockchain, is primarily due to the explosive growth of  numerous crypocurrencies, there are many applications of this core technology that are outside the financial industry.  These applications arise from leveraging various useful features provided by distributed ledgers such as a  decentralized information management,  immutable record keeping for possible audit trail, a robustness and available system,  and  a system that provides security and privacy.  For example, one rapidly emerging area of application of distributed ledger technology is medical and health care. At a high level, the distributed ledger can be used as a platform to store health care data for sharing, recording, analysis, research, etc. One of the most widely discussed approaches in adopting DLT is to implement Health Information Exchange (HIE), for %\nnrev{transactions}{
sharing information among the participants such as patients, caregivers and other relevant parties~\cite{DLT:health:2017}. Another interesting open-source initiative is Namecoin  that uses  DLT to improve the registration and ownership transfer of internet components such as DNS~\cite{Namecoin}. Recently, in the real estate space there has been some experimental study to use DLT to implement a transparent and  decentralized public ledger for managing  land information, where the land registry serves  property rights and historical transactions.  Moreover, such an application would benefit from: $(i)$ time stamping of transactions (a substitute for notarization), $(ii)$ fault-tolerance  from individual  component crashes (as the system does not rely on a single centralized system), and  $(iii)$ non temper-able  %\nnrev{ledger of}{} 
historical transactions and %\nnrev{other  blockchain applications to manage}{} 
registry details~\cite{DLT:RealEstate:2017}. Another example is to apply DLT in the management of scientific research projects to track and manage information such as publications, funding, and analysis in a publicly available, in a reproducible and transparent manner~\cite{DLT:Science}.


In the light of these works 
%We do believe that 
indeed crypto-currencies and (public and private) distributed ledgers\footnote{We will use distributed ledger from now on, instead of blockchain.} 
have the potential to impact our society deeply. 
However, most experts often do not clearly differentiate between the coin, the ledger that supports it, and the service they provide.
%However, when talking with most experts they tend to almost immediately get very technical, 
Instead, they get very technical, talking about the cryptography involved, the mining used to maintain the ledger, or the smart contract technology used. 
Moreover, when asked for details it is often the case that there is no formal specification of the protocols, algorithms, and service provided, with a few exceptions \cite{wood2014ethereum}. In many cases ``the code is the spec.''


From the theoretical point of view there are many fundamental questions with the current distributed ledger 
(and crypto-currency) systems that are very often not properly answered:
%\begin{itemize}
%\item 
What is the service that must be provided by a distributed ledger?
%\item
What properties a distributed ledger must satisfy?
%\item
What are the assumptions made by the protocols and algorithms on the underlying system?
%\item
Does a distributed ledger require a linked crypto-currency?
%\end{itemize}
%
	%We are not the first noticing these issues in the ``blockchain universe.''
	In his PODC'2017 keynote address, Maurice Herlihy pointed out that, despite the hype about
	blockchains and distributed ledgers, no formal abstraction of these objects has been proposed \cite{DBLP:conf/podc/Herlihy17}. He stated that there is a need for the formalization of the distributed systems that are at the heart of most cryptocurrency implementations, and leverage the decades of experience in the distributed computing community in formal specification when designing and proving various properties of such systems. In particular, he noted that the distributed ledger can be formally described by its sequential specification. Then, by using well-known concurrent objects, like consensus objects, come up with a universal construction of linearizable distributed ledgers.%\vspace{-\bigskipamount}


\begin{figure}[t]
	\begin{multicols}{2}
		\begin{algorithm}[H]
			\caption{\small Ledger Object $\ledger$}
			\label{alg:cdl}
			\begin{algorithmic}[1]
				\State \textbf{Init:} $S \leftarrow \emptyset$%\vspace{-1em}
				%			\Statex
				\Function{$\ledger$.\act{get}}{~}
				\State \textbf{return} $S$ %\vspace{-1em}
				\EndFunction
				%			\Statex
				\Function{$\ledger$.\act{append}}{r}
				\State $S \leftarrow S \extends r$
				\State \textbf{return}\vspace{-.8em}
				\EndFunction
				\Statex
			\end{algorithmic}
		\end{algorithm}
		\begin{algorithm}[H]
			\caption{\small Validated Ledger Object $\vledger$} %(only $\act{append}$)}
			\label{alg:vcdl}
			\begin{algorithmic}[1]
				\State \textbf{Init:} $S \leftarrow \emptyset$%\vspace{-1em}
				%			\Statex
				\Function{$\vledger$.\act{get}}{~}
				\State \textbf{return} $S$ %\vspace{-1em}
				\EndFunction
				%
				\Function{$\vledger$.\act{append}}{r}
				\If {$\mathit{Valid}(S \extends r)$}
				\State $S \leftarrow S \extends r$
				\State \textbf{return {\sc ack}}
				\Else ~~\textbf{return {\sc nack}}
				%\State \indent $\ledger \leftarrow \ledger$
				%			\State \indent
				\EndIf 
				\EndFunction
				%\Statex
			\end{algorithmic}
		\end{algorithm}
	\end{multicols}\vspace{-\bigskipamount}%\vspace{-\bigskipamount}
	%\caption{Basic operations of the Ledger Object and its Validated variation.}
\end{figure}


%Moving in this direction, i
In this paper we provide a proper formulation of a family of \emph{ledger objects},
starting from a centralized, non replicated ledger object, and moving to distributed, concurrent 
implementations of ledger objects, subject to validation rules. 
In particular, we provide definitions and sample implementations for the following types of ledger objects:

\begin{itemize}
	\item{\bf Ledger Object (LO):} We begin with a formal definition of a \emph{ledger object}
	as a sequence of \emph{records}, supporting two basic operations: $\act{get}$ and  $\act{append}$. 
	In brief, the ledger object is captured by Code~\ref{alg:cdl} (in which $\extends$ is the concatenation operator), where the $\act{get}$ operation returns the 
	ledger as a sequence $S$ of records, and the $\act{append}$ operation adds a new 
	record at the end of the sequence. 
	The \textit{sequential specification} of the object is then presented, to explicitly define the 
	expected behavior of the object when accessed sequentially by $\act{get}$ and $\act{append}$ operations. 
	
	\item{\bf Distributed Ledger Object (DLO):} With the ledger object implemented on top of multiple 
	(possibly geographically dispersed) \emph{computing devices} or \emph{servers} we
	obtain \emph{distributed ledgers} -- the main focus of this paper. Distribution allows a (potentially very large)
	set of distributed \emph{client processes} to access the distributed ledger, by issuing $\act{get}$ and $\act{append}$
	operations concurrently. To explain the behavior of the operations during concurrency we define 
	three consistency semantics: $(i)$ eventual consistency, $(ii)$ sequential consistency, and $(iii)$ atomic consistency. The definitions provided are
	independent of the properties of the underlying system and the failure model.
	%\ch{[[CG: Should we briefly mention the equivalence to consensus?]]}
	
	\item {\bf Implementations of DLO:}
	In light of our semantic definitions, we provide a number of algorithms that implement DLO that satisfy
	the above mentioned consistency semantics, on asynchronous message passing crash-prone systems, utilizing an Atomic Broadcast service. 
	%Existing distributed structure implementations such as Atomic Broadcast are utilized in our algorithms
	%.\ch{[[CG: We not say explicitly that we use atomic broadcast?]]} 
	
	\item{\bf Validated (Distributed) Ledger Object (V[D]LO):} We then provide a variation of the ledger object -- the \emph{validated ledger object} -- 
	which requires that each record in the ledger satisfies a particular \textit{validation rule}, 
	%The validation rule is 
	expressed as a predicate $\mathit{Valid}()$. 
	%that determines if a sequence of records is in fact valid or not.
	To this end, the basic $\act{append}$ operation of this type of ledger filters each record 
	through the $\mathit{Valid}()$ predicate before is appended to the ledger (see Code~\ref{alg:vcdl}).
\end{itemize}

\noindent{\bf Other related work.}
A distributed ledger can be used to implement a replicated state machine~\cite{lamport1978time,schneider1990implementing}. Paxos~\cite{L98}
is one the first proposals of a replicated state machine implemented with repeated consensus instances. The Practical Byzantine Fault Tolerance solution of Castro and Liskov~\cite{castro2002practical} is proposed to be used in Byzantine-tolerant blockchains. In fact, it is used by them to implement an asynchronous replicated state machine~\cite{castro2000proactive}. The recent work of Abraham and Malkhi~\cite{abraham2017blockchain} discusses in depth the relation  between BFT protocols and  blockchains consensus protocols. 
All these suggest that at the heart of implementing a distributed ledger object there is a version of a consensus mechanism, which directly impacts the efficiency of the 
implemented DLO. In a later section, we show that an eventual consistent DLO can be used to implement consensus, and consensus can be used to implement an
\nn{eventual consistent} DLO; this reinforces the relationship identified in the above-mentioned works.
%\kmk{
%	At the heart of implementing a distributed ledger object is a consensus mechanism, which directly impacts the effeciency of the 
%	implemented DLO. In a later section, with a simple argument that an implementation of a consensus object can be used to implement a DLO. Most practical use of DLOs, at the very least, is on an asynchronous network where the autonomous can fail. 
%	Unfortunately, consensus algorithms that can guarantee liveness and safety  under an asynchrony with crash failures cannot be designed.  One of the simplest forms of component failure is crash failure, where the process stops taking further steps; on the other extreme is the \emph{Byzantine} failure, where the nodes might behave arbitrary ways such as deviate from the protocols they are suppose to execute. One of the earliest algorithm for solving consensus is Paxos\cite{L98}, which works for nodes that can crash fail. Under Byzantine failures the  PBFT by Castro and Likov \cite{castro2002practical} solves consensus, where up to one third of the nodes can experience Byantine failures. 

Among the proposals for distributed ledgers, Algorand~\cite{gilad2017algorand} is an algorithm for blockchain that boasts much higher throughput than Bitcoin and Ethereum.
This work is a new resilient optimal Byzantine consensus algorithm targeting consortium blockchains. To this end, it first revisits the consensus validity property by requiring that the decided value
satisfies a predefined predicate, which does not systematically exclude a value proposed only by Byzantine processes, thereby generalizing the validity properties found in the literature. 
Gramoli et al.~\cite{gramoli2017blockchain, DBLP:journals/corr/CrainGLR17} propose blockchains implemented using Byzantine consensus algorithms that also relax the validity property of the commonly defined consensus problem.
%\af{
In fact, this generalization of the valid consensus values was already introduced by Cachin et al.~\cite{DBLP:conf/crypto/CachinKPS01} as \emph{external validity}.
%In Gramoli's Red Belly system~\cite{gramoli2017blockchain, gramoli2017securing}, a blockchain is implemented on top of a modular Byzantine consensus algorithm that also relaxes the validity property of the commonly defined consensus problem.

%[[\ch{Write about Hyperledger}]]
%\nn{
On the most recent horizon, Linux Foundation initiated the project \emph{Hyperledger} \cite{Hyperledger}.
 Their focus is on developing a modular architectural framework for enterprise-class distributed ledgers. This includes identifying common and
critical components, providing a functional decomposition of an enterprise blockchain stack
into component layers and modules, standardizing interfaces between the components,
and ensuring interoperability between ledgers. The project currently encapsulates five different distributed ledger 
implementations (with coding names Burrow, Fabric, Iroha, Sawtooth, and Indy), each targeting a separate goal. 
%\af{
It is interesting that Fabric~\cite{DBLP:conf/eurosys/AndroulakiBBCCC18}, \nn{although quite different from our work since its objective is to provide an open-source software system, does have} some similarities, like the fact that they use
an atomic broadcast service, the implementation of some level of consistency (in fact, eventual consistency), and 
the fact that it allows the insertion of invalid transactions in the ledger that are filtered out at a later time (as we do in Section~\ref{sec:Valid}).
\nn{However, Fabric does not provide means to achieve stronger consistency, like linearizability or sequential consistency.}
A number of tools are also under development that will allow interaction with the distributed ledgers. Of interest
is the use of tunable, external consensus algorithms by the various distributed ledgers. 

	
%	{\bf And the bitcoin formulation as a register presented in SSS'17. [Will be added]}
One of the closest works to ours is the one by Anceaume et al~\cite{ALPTSSS17}, which like our work, attempts to connect the concept of distributed ledgers with distributed objects,
although they concentrate in Bitcoin. In particular, they first show that read-write registers do not capture Bitcoin's behavior. To this end, they introduce the Distributed Ledger Register (DLR), a register that builds on read-write registers for mimicking the behavior of Bitcoin. In fact, they show the conditions under which the Bitcoin blockchain algorithm satisfies the DLR properties. 
Our work, although it shares the same spirit of formulating and connecting ledgers with concurrent objects (in the spirit of \cite{NFG16}), it differs in many aspects. For example, our formulation does not focus on a specific blockchain (such as Bitcoin), but aims to be more general, and beyond crypto-currencies. Hence, for example, instead of using sequences of blocks (as in~\cite{ALPTSSS17}) we talk about sequences of records. Furthermore, following the concurrent object literature, we define the ledger object on new primitives ($\act{get}$ and $\act{append}$), instead on building on multi-writer, multi-reader R/W register primitives. We pay particular attention on formulating the consistency semantics of the distributed ledger object and demonstrate their versatility by presenting implementations. 
Nevertheless, both works, although taking different approaches, contribute to the better understanding of the basic underlying principles of distributed ledgers from
the theoretical distributed computing point of view. 
} %end remove of Intro

==> linearizability_v1.tex <==
\subsection{Algorithms for Linearizable BDGSOs}

\red{Here, we present an implementation of a linearizable BDGSO. Code~\ref{code:linear-client-BGS} specifies the algorithm run by clients and Code~\Code~\ref{code:ec-server-BGS} specifies the algorithm run by servers. Following, we provide some intuition about how such algorithms behave:}
\begin{itemize}
\item
Intuition of Code~\ref{code:linear-client-BGS}: The claim is that this code, \red{in combination with Code~\ref{code:ec-server-BGS},} implements a linearizable BDGSO, provided $n \geq 4f+1$, where $n$ denotes the number of servers.
\begin{itemize}
\item
\red{Each} $\ledger.\act{add}(r)$ operation is sent to all $n$ servers, which guarantees that at least $n-f$ correct servers \red{will} process it. The operation is considered successful and can complete when at least $n-f$ message acknowledgements have been received. Observe that, \red{since} at least $n-2f>n/2$ of these servers are correct, this implies that when the $\ledger.\act{add}(r)$ operation completes, a majority of the servers have $r$ in their sets.

\item
\red{Each} $\pi=\ledger.\act{get}()$ operation requests their set to all the $n$ servers, out of which we know at least $n-f$ will reply (since they are correct). Let $R$ be the set of \ar{servers who have sent} the first $n-f$ responses received. Consider any record $r$ whose $\pi'=\ledger.\act{add}(r)$ operation completed before $\pi$ started. Let $A$ be the set of at least $n-2f$ correct servers whose ACK was received in the processing of $\pi'$. We have that $|R \cap A| \geq n-3f \geq f+1$. Hence, $r$ will be included in
at least $n-3f$ of the sets $S_i$ received from the servers, and will be in the set $S$ returned by $\pi$.
\end{itemize}

\item 
\red{Intuition of Code~\ref{code:ec-server-BGS}: In this algorithm and in order to prevent spurious records to be inserted by Byzantine clients, it is assumed that up to $t$ clients can be Byzantine. So, the set $S_i$ contains the records that have been added by at least $t+1$ clients.}

The BRB service guarantees that any record added by a correct server $i$ to $S_i$ will be eventually added by all correct servers $j$ in their respective sets $S_j$.

\end{itemize}


\setlength{\columnsep}{10pt}
\begin{figure}[t]
%	\begin{multicols}{2}
		%\begin{wrapfigure}{R}{0.43\textwidth}
		%	\begin{minipage}{0.43\textwidth}\vspace{-2em}
		\begin{algorithm}[H]
			\caption{\small Client API and algorithm for Linearizable Byzantine-tolerant Distributed G-Set Object $\ledger$, for $n \geq 4f+1$ servers}
			\label{code:linear-client-BGS}
			%	\begin{multicols}{2}
			\begin{algorithmic}[1]
    				\State  \textbf{Init:} $c \leftarrow 0$
    				\Function{$\ledger.\act{get}$}{~}
    				\State $c \leftarrow c + 1$
    			        	\State
                             {\bf send} request ($c$, $p$, {\sc get}) $4f+1$ different servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc getResp}, $S_i$) from $3f+1$ different servers \label{c5-L5}
    				\State $S \leftarrow \{r:$ record $r$ is in at least $f+1$ sets $S_i \}$ \label{c5-L6}
    				\State \textbf{return} $S$
    				\EndFunction
    				\Function{$\ledger.\act{add}$}{$r$}
    				\State $c \leftarrow c + 1$
    				\State \textbf{send} request ($c$, $p$, {\sc add}, $r$) to all servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc addResp}, {\sc ack}) from $n-f$ different servers
    				\State \textbf{return} {\sc ack}
    				\EndFunction
    			\end{algorithmic}
		\end{algorithm}
\end{figure}

\setlength{\columnsep}{10pt}
\begin{figure}[t]
%	\begin{multicols}{2}
		%\begin{wrapfigure}{R}{0.43\textwidth}
		%	\begin{minipage}{0.43\textwidth}\vspace{-2em}
		\begin{algorithm}[H]
			\caption{\small \af{Client API and algorithm for Linearizable Byzantine-tolerant Distributed G-Set Object $\ledger$, for $n \geq 4f+1$ servers, VERSION AF}}
			\label{code:linear-client-BGS}
			%	\begin{multicols}{2}
			\begin{algorithmic}[1]
    				\State  \textbf{Init:} $c \leftarrow 0$
    				\Function{$\ledger.\act{get}$}{~}
    				\State $c \leftarrow c + 1$
    			        	\State
                             {\bf send} request ($c$, $p$, {\sc get}) all $n$ servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc getResp}, $S_i$) from $n-f$ different servers \label{c5-L5}
    				\State $S \leftarrow \{r:$ record $r$ is in at least $f+1$ received sets $S_i \}$ \label{c5-L6}
    				\While{($|\{i: S \subseteq S_i\}|  < n-2f$)}
    				    \State {\bf send} request ($c$, $p$, {\sc get}) all $n$ servers
    				    \State \textbf{wait} responses ($c$, $i$, {\sc getResp}, $S_i$) from $n-f$ different servers
    				\EndWhile
    				\State \textbf{return} $S$
    				\EndFunction
    				\Function{$\ledger.\act{add}$}{$r$}
    				\State $c \leftarrow c + 1$
    				\State \textbf{send} request ($c$, $p$, {\sc add}, $r$) to all servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc addResp}, {\sc ack}) from $n-f$ different servers
    				\State \textbf{return} {\sc ack}
    				\EndFunction
    			\end{algorithmic}
		\end{algorithm}
\end{figure}


\setlength{\columnsep}{10pt}
\begin{figure}[t]
	\begin{algorithm}[H]
			\caption{\small Server algorithm for both Linearizable and Eventual Consistent Byzantine-tolerant Distributed G-Set Object}
			\label{code:ec-server-BGS}
			\begin{algorithmic}[1]
				\State \textbf{Init:} $S_i \leftarrow \emptyset$
				\Receive{{\sc get}($c$, $p$)} 
				\State \textbf{send} response {\sc getResp}($c$, $i$, $S_i$) to $p$ \label{C4-L03}
				\EndReceive
				
				\Receive{{\sc add}($c$, $p$, $r$)} \af{[[AF: The signature of $p$ is validated]]}
				\If{($r \notin S_i$)} 
				\State \act{BRB-broadcast}({\sc propagate}($i$, {\sc add}($c$, $p$, $r$))) \label{C4-L06}
				\State \textbf{wait until} $r \in S_i$ \label{C4-L07}
				\EndIf
				\State  \textbf{send} response {\sc addResp}($c$, $i$, {\sc ack}) to $p$
				\EndReceive
				\Upon{\act{BRB-deliver}({\sc propagate}($j$, {\sc add}($c$, $p$, $r$)))} \af{[[AF: The signatures of $j$ and $p$ are validated]]} \label{C4-L09}
				\If{($r \notin S_i$) and ({\sc add}($c$, $p$, $r$) was received from $f+1$ different servers $j$)} \label{C4-L10}
				\State $S_i \leftarrow S_i  \cup \{r\}$ \label{C4-L11}
				\EndIf
				\EndUpon
			\end{algorithmic}
		\end{algorithm}
\end{figure}

\setlength{\columnsep}{10pt}
\begin{figure}[t]
%	\begin{multicols}{2}
		%\begin{wrapfigure}{R}{0.43\textwidth}
		%	\begin{minipage}{0.43\textwidth}\vspace{-2em}
		\begin{algorithm}[H]
			\caption{\small \af{Client API and algorithm for Linearizable Byzantine-tolerant Distributed G-Set Object $\ledger$, for $n \geq 4f+1$ servers, VERSION AF}}
			\label{code:linear-client-BGS}
			%	\begin{multicols}{2}
			\begin{algorithmic}[1]
    				\State  \textbf{Init:} $c \leftarrow 0$
    				\Function{$\ledger.\act{get}$}{~}
    				\State $c \leftarrow c + 1$
    			        	\State
                             {\bf send} request ($c$, $p$, {\sc get}) all $n$ servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc getResp}, $S_i$) from $n-f$ different servers \label{c5-L5}
    				\State $S \leftarrow \{r:$ record $r$ is in at least $f+1$ received sets $S_i \}$ \label{c5-L6}
    				\While{($|\{i: S \subseteq S_i\}|  < n-2f$)}
    				    \State {\bf send} request ($c$, $p$, {\sc get}) all $n$ servers
    				    \State \textbf{wait} responses ($c$, $i$, {\sc getResp}, $S_i$) from $n-f$ different servers
    				\EndWhile
    				\State \textbf{return} $S$
    				\EndFunction
    				\Function{$\ledger.\act{add}$}{$r$}
    				\State $c \leftarrow c + 1$
    				\State \textbf{send} request ($c$, $p$, {\sc add}, $r$) to all servers
    				\State \textbf{wait} responses ($c$, $i$, {\sc addResp}, {\sc ack}) from $n-f$ different servers
    				\State \textbf{return} {\sc ack}
    				\EndFunction
    			\end{algorithmic}
		\end{algorithm}
\end{figure}

\setlength{\columnsep}{10pt}
\begin{figure}[t]
	\begin{algorithm}[H]
			\caption{\small \nn{Server algorithm for both Linearizable and Eventual Consistent Byzantine-tolerant Distributed G-Set Object: VERSION NN}}
			\label{code:ec-server-BGS}
			\begin{algorithmic}[1]
				\State \textbf{Init:} $S_i \leftarrow \emptyset$
				\Receive{{\sc get}($c$, $p$)} 
				\State \act{BRB-broadcast}({\sc propagate}($i$, $S_i$))
				\State \textbf{wait until} $2f+1$ servers respond
				\State \textbf{send} response {\sc getResp}($c$, $i$, $S_i$) to $p$ \label{C4-L03}
				\EndReceive
				
				\Receive{{\sc add}($c$, $p$, $r$)} \af{[[AF: The signature of $p$ is validated]]}
				\If{($r \notin S_i$)} 
				\State \act{BRB-broadcast}({\sc propagate}($i$, {\sc add}($c$, $p$, $r$))) \label{C4-L06}
				\State \textbf{wait until} $r \in S_i$ \label{C4-L07}
				\EndIf
				\State  \textbf{send} response {\sc addResp}($c$, $i$, {\sc ack}) to $p$
				\EndReceive
				\Upon{\act{BRB-deliver}({\sc propagate}($j$, {\sc add}($c$, $p$, $r$)))} \af{[[AF: The signatures of $j$ and $p$ are validated]]} \label{C4-L09}
				\If{($r \notin S_i$) and ({\sc add}($c$, $p$, $r$) was received from $f+1$ different servers $j$)} \label{C4-L10}
				\State $S_i \leftarrow S_i  \cup \{r\}$ \label{C4-L11}
				\EndIf
				\EndUpon
				\Upon{\act{BRB-deliver}({\sc propagate}($j$, $S_j$)} \nn{[[NN: The signature of $j$ is validated]]} \label{C4-L09}
				\State {\bf wait until} $S_j \subseteq S_i$ \label{C4-L15e}
				\State \textbf{send} response {\sc setResp}($S_j$) to $j$ \label{C4-L03}
				\EndIf
				\EndUpon
			\end{algorithmic}
		\end{algorithm}
\end{figure}

\begin{lemma}
\label{lemma:linear-causality}
Codes~\ref{code:linear-client-BGS} and~\ref{code:ec-server-BGS} guarantee that $\forall r$ returned by a $\pi = \ledger.\act{get}() \in \hist{\ledger}$, an $\ledger.\act{add}(r)$ invocation precedes $\pi$ response in  $\hist{\ledger}$
\end{lemma}
\begin{proof}
Let $S$ be the set returned by $\pi$. $\forall r \in S$, client collects $f+1$ (-, -, {\sc getResp}, $S_i$) containing $r$ (Line~\ref{C4-L06} of Code~\ref{code:linear-client-BGS}). So at least a correct server has $r$ in its local set $S_i$;  a correct server adds a record to its local set only when it has received $f+1$ {\sc propagate}(-, {\sc add}($c$, -, $r$)) from different servers. Since at least one is correct, then $\ledger.\act{add}(r)$ invocation is ensured to have happened at least on one server; so it happened and preceded $\pi$ response in $\hist{\ledger}$. 
\end{proof}


\begin{theorem} Codes~\ref{code:linear-client-BGS} and~\ref{code:ec-server-BGS} implement a linearizable  BDGSO, where up to $f$ out of $n \geq 4f+1$ servers can be Byzantine.
\end{theorem}

\begin{proof}
We need to demonstrate that Codes~\ref{code:linear-client-BGS} and~\ref{code:ec-server-BGS} guarantee Byzantine Completeness ({\em BC}) and Byzantine Linearizability ({\em BL}).
\begin{itemize}
\item 
{\em BC:} $\ledger.\act{get}()$ algorithm sends requests to all servers and since server simply return its local $S_i$ set, client eventually receives at least $n-f$ responses. Also $\ledger.\act{add}()$ sends requests to all servers, so at least all $n-f$ correct ones will call BRB-Broadcast; by BRB-Validity and BRB-Termination all correct servers receives at least $n-f\geq3f+1$ so line 10 of Code~\ref{code:ec-server-BGS} is unlocked and client receives at least $n-f$ responses.
%
\item
{\em BL:} Proof of Byzantine Linearizability implies to demonstrate that shown algorithms respect sequential specification in Definition~\ref{def:sspec} in respect to a an $\ledger.\act{add}(r)$ followed by a $\ledger.\act{get}()$ and to two subsequent $\ledger.\act{get}()$. For this point will be enough to demonstrate that once an $\ledger.\act{add}(r)$ successfully returns on a correct client, then all subsequent $\ledger.\act{get}()$ will definitely have $r \in S$. Moreover it is necessary to show that $\ledger.\act{get}()$ only include records previously added following the $\ledger.\act{add}(r)$ algorithm.

Consider a \nn{[NN: what is the arrow notation?]}$S \leftarrow \pi'=\ledger.\act{get}()$ issued, by a correct client, right after a $\pi=\ledger.\act{add}(r)$. If we demonstrate that $S$ must include $r$ then we are done because local $S_i$ sets of all correct servers can only grow with the {\em Union} operator in Line~\ref{C4-L11}

Client running the $\ledger.\act{add}(r)$ algorithm sends requests to all servers and waits for $n-f$ acknowledgements ($c$, -, {\sc addResp}, {\sc ack}) from different servers that means at least $n-2f$ correct servers successfully added $r$ to their local $S_i$ set. For Byzantine Completeness, just demonstrated, this eventually always happens.

($c$, -, {\sc get}) requests of $\pi'$ are sent by client to $4f+1$ servers and $3f+1$ ($c$, -, {\sc getResp}, $S_i$) are awaited to continue execution. Let us consider the worst case in which all $3f+1$ responses include $f$ byzantine server responses and $f$ responses from server who did not acknowledged $\pi$. This anyway means that there are $f+1$ responses from correct servers who acknowledged $\pi$, so condition in Line~\ref{c5-L6} is satisfied and $r \in S$. We have shown that $\ledger.\act{add}(r) \rightarrow \ledger.\act{get}()$ implies $r \in S$ with $S$ being $\ledger.\act{get}()$ answer.

We need to demonstrate that if $\pi = \ledger.\act{get}() \rightarrow \pi' = \ledger.\act{get}()$ in a generic permutation $\sigma$ then sequential specification is respected. Say $S$ set returned by $\pi$ and $S'$ set returned by $\pi'$. Assume sequential specification for $\pi$ and $\pi'$ is not respected, so $\exists r \in S: r \notin S'$. For Lemma~\ref{lemma:linear-causality} we know that a $\pi'' = \ledger.\act{add}(r)$ invocation exists and happened before $\pi$ response. This implies, since we are considering a generic permutation $\sigma$, that $\pi'' \rightarrow \pi$ in $\sigma$;\nn{[NN: this is not true! You consider the order of events and not the order of operations! saying that the invocation of $\pi''$ happened before the response of $\pi$ does not mean that the response of $\pi''$ happened before the invocation of $\pi$ (which is needed in order to say $\pi''\rightarrow\pi$]} \ar{[AR: I agree with what you say, but in respect to $\hist{\ledger}$ not in respect to a permutation $\sigma$. Since $\sigma$ in Def. 2 is only constrained on operations, does this not mean that we can put the Add response event wherever, so, also before the two Gets ? We're stating that a permutation exists, not that property holds for all permutations.]}\nn{[NN: The before than relation $\rightarrow$ should hold on real time ordering of operations]} by hypothesis we know that $\pi \rightarrow \pi'$ so necessarily $\pi'' \rightarrow \pi'$. For what we just demonstrated, $\ledger.\act{add}(r) \rightarrow \ledger.\act{get}()$ implies $r$ returned by $\ledger.\act{get}()$ answer, so $r \in S'$; result is that $\pi$ and $\pi'$ respect the sequential specification but this contradicts our initial assumption.\ar{AR: I think you're true, because response of add is not ensure to have happened at all and may not exist.}\nn{[This is true! :) Without ensuring that the add(r) operation terminates before both gets() then you cannot guarantee that both of them will discover the element $r$ in $f+1$ servers. The easy fix is to have the get() operation to propagate $S$ to $2f+1$ servers before returning.]}\ar{[[AR: We should ensure that if a get sees a record also the subsequent one does. I think is enough to raise threshold of f+1 in line 10 to the majority of servers.]]}\nn{[NN: No it is not! The problem will accumulate as you have multiple (non-concurrent) get() operations concurrent with a single add() operation]}\nn{[You mean line 10 in Alg 2?] }\ar{[AR: yes]}\nn{[NN: hmm...this may solve the issue if we wait for 2f+1...indeed...hmm how do you ensure though that once f+1 servers add it in their S then all 2f+1 servers will also do? Still problematic...you should apply the BRB during the get() operation if you want to use that method.]}
\ar{[AR: yes, it does not seem to solve the problem without making other modifications.]}\ar{[AR: What about raising thresholds in lines 4/5/6 of Alg. 1 to the majority of server.]}\nn{[As i said before the problem will accumulate when you have more than 2 get() operations. Say that you wait for 3f+1. Then you may see $r$ in $2f+1$ then next get() might see $r$ in $f+1$.]}\ar{[AR: Assume $n$ in line 4, $n-f$ in line 5 and $2f+1$ in line 6]}\nn{[What is $n$? $n>4f+1$?]}\ar{[AR: Yes, maybe we have to raise it]}\ar{[AR: I think there still is problem of accumulation you were mentioning and this is not a good way to provide a solution. Even considering $n-2f$ in line 6 for the Get().]}\nn{[NN: I would say that the most elegant solution is to have the servers perform a BRB with their local $S$ and wait for $2f+1$ deliveries before replying to the get() operation.]}
% Demo with Get() sending to all servers
%$\pi_2$ requests are sent to all servers, too, and client waits for $n-f$ confirmations. This implies that, in general, $n-2f$ correct server responding to $\pi_1$ must intersect at least $n-3f$ servers responding to $\pi_2$. Since we assume $n \geq 4f+1$ then at least $f+1$ correct server responses, who acknowledged $r$ in their local $S_i$ sets, will be counted by clients and $r$ will be returned in $S$. Since we did not assume anything on which servers are answering to $\pi_1$ and $\pi_2$ then what just stated is valid for any $\ledger.\act{add}(r) \rightarrow \ledger.\act{get}()$.%
\end{itemize}
\end{proof}
